RMFlow: Refined Mean Flow by a Noise-Injection Step for Multimodal Generation

Mean flow (MeanFlow) enables efficient, high-fidelity image generation, yet its single-function evaluation (1-NFE) generation often cannot yield compelling results. We address this issue by introducing RMFlow, an efficient multimodal generative model that integrates a coarse 1-NFE MeanFlow transport with a subsequent tailored noise-injection refinement step. RMFlow approximates the average velocity of the flow path using a neural network trained with a new loss function that balances minimizing the Wasserstein distance between probability paths and maximizing sample likelihood. RMFlow achieves near state-of-the-art results on text-to-image, context-to-molecule, and time-series generation using only 1-NFE, at a computational cost comparable to the baseline MeanFlows.

==> proof.tex <==

\vspace{-0.2cm}
\subsection{Model Training}\label{subsec:model-training}
\vspace{-0.2cm}
We now present a new loss function to balance mean flow matching and likelihood maximization.

\BW{$t=r$} 

\SW{Derive: if there is a KL control, DDIM's equations 57 and C.2.}
\subsubsection{Mean Flow Matching: Geometric Control}
\SW{Check the novelty again with Yuhao, if these are borrowed from existing works moved to Background}
We perform mean flow matching by minimizing the loss function $\gL_{\rm CMFM}(\theta)$ in \eqref{eq:mean-flow-matching}.


A foundational result for FM is that $\nabla_\theta\gL_{\rm CFM}(\theta)=\nabla_\theta\gL_{\rm FM}(\theta)$, where $\gL_{\rm CFM}(\theta)$ is in \eqref{eq:CFM} and $\gL_{\rm FM}(\theta):=\mathbb{E}_{t,p_t(\vx)}[\|\hat{\vu}_t(\vx;\theta)-\vu_t(\vx)\|^2]$ (cf.~\cite[Theorem 2]{lipman2022flow}). However, such a result has not been established for $\gL_{\rm CMFM}$; in response, we establish it as follows: 
\begin{restatable}{theorem}. \label{th:equiv_bp}
We have
\begin{equation}
\nabla_\theta \gL_{\rm CMFM}(\theta)=\nabla_\theta\gL_{\rm MFM}(\theta),
\end{equation}
where $\gL_{\rm CMFM}(\theta)$ is defined in \eqref{eq:mean-flow-matching} and $\gL_{\rm MFM}$ is obtained by replacing $\vu_{t,r}^{\rm tgt}(\vx;\theta^*)$ with $\vu_t(\vx) + (r-t)\big[ \nabla\hat{\vu}_{t,r}(\vx;\theta^*)\cdot\vu_t(\vx) + \partial_t\hat{\vu}_{t,r}(\vx;\theta^*) \big]$ in $\gL_{\rm CMFM}$.
\end{restatable}
Theorem~\ref{th:equiv_bp} guarantees equivalence in learning $\hat{\vu}_{t,r}(\vx;\theta)$ between minimizing $\gL_{\rm CMFM}(\theta)$ and $\gL_{\rm MFM}(\theta)$. We remark that {\bf stop gradient is essential for establishing this result}.




As the second theoretical contribution, we prove that minimizing $\gL_{\rm CMFM}(\theta)$ can effectively reduce the Wasserstein distance between the probability flows induced by the ground truth mean velocity $\vu_{r,t}$ and its neural network approximation $\hat{\vu}_{r,t}$. Due to the fact that minimizing $\gL_{\rm CMFM}(\theta)$ controls the distance between the probability flows, we name it {\bf geometric control}. In particular, we have
\BW{[Mention that our theorem is inspired by the analysis of N. Boffi et al's work. Then, stress what is the key novelty of our result]}


%\BW{[LLM: (Refs) Why do we analyze the Wasserstein distance? geometric distance] Perhaps this paper \url{https://www.arxiv.org/pdf/2508.03210}} \BW{[Dynamical path: why Wasserstein]}




% \begin{restatable}[Flow Map]{definition}. By reparameterization, we define the following flow map $\bm{\Psi}_{t,r}: \sR^n\rightarrow\sR^n$ for the ODE in~\eqref{eq:lrg_flow_ODE}:
% \begin{equation}
% \bm{\Psi}_{t,r}(\vx_t) = \vx_t + (r-t)\vu_{t,r}(\vx_t) = \vx_r,\quad\text{for all }(t,r)\in[0,1]^2
% \end{equation}
% and the learned flow map:
% \begin{equation}
% \bm{\hat\Psi}_{t,r}(\vx_t) = \vx_t + (r-t)\hat\vu_{t,r}(\vx_t;\theta) = \hat\vx_r,\quad\text{for all }(t,r)\in[0,1]^2
% \end{equation}
% where $\hat \vx_r$ denotes a generated sample and $\vx_t$ is any solution to~\eqref{eq:lrg_flow_ODE}.
% \end{restatable}

\SW{$p_{t,r}:=p\big(\vx_t + (t-r)\vu_{t,r}(\vx_t)\big)$ is not a valid notation.}
\begin{restatable}[Wasserstein distance between probability flows]{theorem}.\label{th:wasser} 
Let $p_{t,r}:=p\big(\vx_t + (t-r)\vu_{t,r}(\vx_t)\big)$ and $\hat p_{t,r}=\hat p\big(\vx_t + (t-r)\hat\vu_{t,r}(\vx_t;\theta)\big)$ be the probability flow induced by the exact ($\vu_{t,r}(\vx_t)$) and approximated $\hat\vu_{t,r}(\vx_t;\theta)$ mean velocity, respectively. Then the Wasserstein distance, $W_2^2(p_{t,r},\hat p_{t,r}):=\inf_{\gamma\in \prod(p_{t,r},\hat p_{t,r})}\int_{\mathbb{R}^d\times \mathbb{R}^d}\|\vx-\vy\|^2 d\gamma(\vx,\vy)$ with $\prod(p_{t,r},\hat p_{t,r})$ being the joint distribution of $p_{t,r}$ and $\hat{p}_{t,r}$, between $p_{t,r}$ and $\hat{p}_{t,r}$ satisfies \BW{[double check notations]}
\begin{equation}
\begin{aligned}
W_2^2(p_{t,r}, \hat p_{t,r})&\leq \int_t^r\exp{(s-t)}\E_{p_s(\vx)}\big[\big\|\hat\vu_{t,r}(\vx;\theta) - \vu_{t,r}^{\rm tgt}(\vx;\theta^*)\big\|^2\big]ds\\
&\BW{\leq 2.72\gL_{\rm MFM}},
\end{aligned}
\end{equation} 
and
\begin{equation}
W_2^2(p_{0,r},\hat p_{0,r}) \leq \E_{p(t|r),p_t(\vx)}\Big[\frac{\exp{(t)}}{p(t|r)}
%\bm\varepsilon_{t,r}(\vx;\theta,\theta^{-})
\big\|\hat\vu_{t,r}(\vx;\theta) - \vu_{t,r}^{\rm tgt}(\vx;\theta^*)\big\|^2
\Big].
\end{equation}
\end{restatable}
%\BW{[Remarks on the upper bound]}
\BW{Remark: minimizing CMFM equivalents to minimizing MFM, and Theorem 3.2 is based on MFM. Remark on why the error is bounded if the loss is small.}


\vspace{-0.2cm}



\subsection{Equivalence of Objectives}\label{sec:equiv_loss}
\textcolor{blue}{TODO: modify the symbols}
In this section, we prove 
\begin{equation}
\nabla_{\theta}\gL_{\rm SMFI}(\theta;\theta^{-})=\nabla_{\theta}\gL_{\rm CSMFI}(\theta;\theta^{-})  
\end{equation}
in backpropagation. \texttt{stopgrad} operator plays an important role for the unbiased estiation of the gradient w.r.t. model parameters in backpropagation.

By expanding $\gL_{\rm SMFI}$ in~\eqref{eq:loss_mfsi}, and taking gradient w.r.t. $\theta$, we have:
\begin{equation}\label{eq:grad_mfsi}
\begin{aligned}
&\nabla_{\theta}\gL_{\rm SMFI}(\theta;\theta^{-})=\\
&\iiint p_t(\vx)\nabla_{\theta}\big\|\hat\vu_{t,r}(\vx;\theta)\big\|^2 d\vx dt dr + \underbrace{\nabla_{\theta}\E_{r,t,p_t(\vx)}\Big[\big\|\vu^{\rm tgt}_{t,r}(\vx;\theta^{-})\big\|^2\Big]}_{=0}  \\
&\hspace{3em}- 2\iiint p_t(\vx)\nabla_{\theta}\big\langle\hat\vu_{t,r}(\vx;\theta), \vu^{\rm tgt}_{t,r}(\vx;\theta^{-})\big\rangle d\vx dt dr \\
&=\iiint p_t(\vx)\nabla_{\theta}\big\|\hat\vu_{t,r}(\vx;\theta)\big\|^2 d\vx dt dr \\
&\hspace{3em} - 2\iiint p_t(\vx)\nabla_{\theta}\big\langle\hat\vu_{t,r}(\vx;\theta), \vu^{\rm tgt}_{t,r}(\vx;\theta^{-})\big\rangle d\vx dt dr \\
&=\iiint\Big[ \iint p_t\big(\vx|\vx_1,\bm\phi_{\omega}(\vc)\big)q\big(\vx_1,\bm\phi_{\omega}(\vc)\big)d\vx_1d\bm\phi_{\omega}(\vc)\cdot\nabla_{\theta}\big\|\hat\vu_{t,r}(\vx;\theta)\big\|^2\Big] d\vx dt dr \\
&\hspace{3em} - 2\iiint p_t(\vx)\big\langle\nabla_{\theta}\hat\vu_{t,r}(\vx;\theta), \vu^{\rm tgt}_{t,r}(\vx;\theta^{-})\big\rangle d\vx dt dr \\
\end{aligned}
\end{equation}
Based on~\eqref{eq:cond_v_p}, we also have:
\begin{equation}\label{eq:inner_cond}
\begin{aligned}
& p_t(\vx)\big\langle\nabla_{\theta}\hat\vu_{t,r}(\vx;\theta), \vu^{\rm tgt}_{t,r}(\vx;\theta^{-})\big\rangle \\
=&  p_t(\vx)\big\langle\nabla_{\theta}\hat\vu_{t,r}(\vx;\theta), \vv_t(\vx)+(r-t)\big[\nabla_{\vx} \hat\vu_{t,r}(\vx;\theta^{-})\cdot\vv_t(\vx) + \partial_{t} \hat\vu_{t,r}(\vx;\theta^{-})\big]\big\rangle \\
=&  p_t(\vx)\big\langle\nabla_{\theta}\hat\vu_{t,r}(\vx;\theta), \big[\mI+(r-t)\nabla_{\vx} \hat\vu_{t,r}(\vx;\theta^{-})\big]\cdot\vv_t(\vx)\big\rangle + p_t(\vx)\big\langle\nabla_{\theta}\hat\vu_{t,r}(\vx;\theta),\partial_{t} \hat\vu_{t,r}(\vx;\theta^{-})\big]\big\rangle \\
=& p_t(\vx)\Big\langle\nabla_{\theta}\hat\vu_{t,r}(\vx;\theta), \big[\mI+(r-t)\nabla_{\vx} \hat\vu_{t,r}(\vx;\theta^{-})\big]\cdot\iint \vv_t\big(\vx\mid\vx_1,\bm\phi_{\omega}(\vc)\big)\frac{p_t\big(\vx|\vx_1,\bm\phi_{\omega}(\vc)\big)q\big(\vx_1,\bm\phi_{\omega}(\vc)\big)}{p_t(\vx)}d\vx_1d\bm\phi_{\omega}(\vc)\Big\rangle \\
&+\iint p_t\big(\vx|\vx_1,\bm\phi_{\omega}(\vc)\big)q\big(\vx_1,\bm\phi_{\omega}(\vc)\big)d\vx_1d\bm\phi_{\omega}(\vc)\big\langle\nabla_{\theta}\hat\vu_{t,r}(\vx;\theta),\partial_{t} \hat\vu_{t,r}(\vx;\theta^{-})\big\rangle \\
=& \iint p_t(\vx)\frac{p_t\big(\vx|\vx_1,\bm\phi_{\omega}(\vc)\big)q\big(\vx_1,\bm\phi_{\omega}(\vc)\big)}{p_t(\vx)}d\vx_1d\bm\phi_{\omega}(\vc)\Big\langle\nabla_{\theta}\hat\vu_{t,r}(\vx;\theta), \big[\mI+(r-t)\nabla_{\vx} \hat\vu_{t,r}(\vx;\theta^{-})\big]\cdot \vv_t\big(\vx\mid\vx_1,\bm\phi_{\omega}(\vc)\big)\Big\rangle \\
&+\iint p_t\big(\vx|\vx_1,\bm\phi_{\omega}(\vc)\big)q\big(\vx_1,\bm\phi_{\omega}(\vc)\big)d\vx_1d\bm\phi_{\omega}(\vc)\big\langle\nabla_{\theta}\hat\vu_{t,r}(\vx;\theta),\partial_{t} \hat\vu_{t,r}(\vx;\theta^{-})\big\rangle \\
=& \iint p_t\big(\vx|\vx_1,\bm\phi_{\omega}(\vc)\big)q\big(\vx_1,\bm\phi_{\omega}(\vc)\big)\Big\langle\nabla_{\theta}\hat\vu_{t,r}(\vx;\theta), \\
& \hspace{16em}\big[\mI+(r-t)\nabla_{\vx} \hat\vu_{t,r}(\vx;\theta^{-})\big]\cdot \vv_t\big(\vx\mid\vx_1,\bm\phi_{\omega}(\vc)\big) + \partial_t \vu_{t,r}(\vx;\theta^{-})\Big\rangle d\vx_1d\bm\phi_{\omega}(\vc)\\
=& \iint p_t\big(\vx|\vx_1,\bm\phi_{\omega}(\vc)\big)q\big(\vx_1,\bm\phi_{\omega}(\vc)\big)\big\langle\nabla_{\theta}\hat\vu_{t,r}(\vx;\theta), \vu^{\rm ctgt}_{t,r}(\vx\mid \vx_1,\bm\phi_{\omega}(\vc);\theta^{-})\big\rangle d\vx_1d\bm\phi_{\omega}(\vc)
\end{aligned}
\end{equation}
by plugging~\eqref{eq:inner_cond} into~\eqref{eq:grad_mfsi}:
\begin{equation}\label{eq:grad_mfsi}
\begin{aligned}
&\nabla_{\theta}\gL_{\rm SMFI}(\theta;\theta^{-})=\\
& \iint\iiint  p_t\big(\vx|\vx_1,\bm\phi_{\omega}(\vc)\big)q\big(\vx_1,\bm\phi_{\omega}(\vc)\big)\cdot\nabla_{\theta}\big\|\hat\vu_{t,r}(\vx;\theta)\big\|^2 d\vx d\vx_1d\bm\phi_{\omega}(\vc) dt dr \\
&-2\iint\iiint p_t\big(\vx|\vx_1,\bm\phi_{\omega}(\vc)\big)q\big(\vx_1,\bm\phi_{\omega}(\vc)\big)\big\langle\nabla_{\theta}\hat\vu_{t,r}(\vx;\theta), \vu^{\rm ctgt}_{t,r}(\vx\mid \vx_1,\bm\phi_{\omega}(\vc);\theta^{-})\big\rangle d\vx d\vx_1d\bm\phi_{\omega}(\vc) dt dr \\
& = \E_{r,t,p_t(\vx|\vx_1,\bm\phi_{\omega}(\vc)),q(\vx_1,\bm\phi_{\omega}(\vc))}\big[\nabla_{\theta}\big\|\hat\vu_{t,r}(\vx;\theta)\big\|^2\big] + 0\\
&\hspace{3em} - 2 \E_{r,t,p_t(\vx|\vx_1,\bm\phi_{\omega}(\vc)),q(\vx_1,\bm\phi_{\omega}(\vc))}\big[\big\langle\nabla_{\theta}\hat\vu_{t,r}(\vx;\theta), \vu^{\rm ctgt}_{t,r}(\vx\mid \vx_1,\bm\phi_{\omega}(\vc);\theta^{-})\big\rangle\big]\\
& = \nabla_{\theta}\E_{r,t,p_t(\vx|\vx_1,\bm\phi_{\omega} (\vc)),q(\vx_1,\bm\phi_{\omega}(\vc))}\big[\big\|\hat\vu_{t,r}(\vx;\theta)\big\|^2\big] \\
&\hspace{1.5em} + \nabla_{\theta}\E_{r,t,p_t(\vx|\vx_1,\bm\phi_{\omega} (\vc)),q(\vx_1,\bm\phi_{\omega}(\vc))}\big[\big\|\vu^{\rm ctgt}_{t,r}(\vx\mid \vx_1,\bm\phi_{\omega}(\vc);\theta^{-})\big\|^2\big]\\
&\hspace{3em} - 2 \nabla_{\theta}\E_{r,t,p_t(\vx|\vx_1,\bm\phi_{\omega}(\vc)),q(\vx_1,\bm\phi_{\omega}(\vc))}\big[\big\langle\hat\vu_{t,r}(\vx;\theta), \vu^{\rm ctgt}_{t,r}(\vx\mid \vx_1,\bm\phi_{\omega}(\vc);\theta^{-})\big\rangle\big] \\
& = \nabla_{\theta}\gL_{\rm CSMFI}(\theta;\theta^{-})
\end{aligned}
\end{equation}
Thus, we have $\nabla_{\theta}\gL_{\rm SMFI}(\theta;\theta^{-})=\nabla_{\theta}\gL_{\rm CSMFI}(\theta;\theta^{-})$ in backpropagation.
\subsection{Wasserstein Bound}\label{sec:w2_bound}
\textcolor{blue}{TODO: modify the symbols}
As discussed in the main paper, $p_t(\vx)$ denotes the probability path of the ODE in~\eqref{eq:lrg_flow_ODE}. Let $\vx_t$ denotes the state variable of the ODE in~\eqref{eq:lrg_flow_ODE}. Then, it is easy to see $\vx_t\sim p_t(\vx)$. Thus, we have
\begin{equation}
\E_{p_t(\vx)}\Big[\big\|\bm{\Psi}_{t,r}(\vx) - \bm{\hat\Psi}_{t,r}(\vx)\big\|^2\Big] = \E_{\vx_t}\Big[\big\|\bm{\Psi}_{t,r}(\vx_t) - \bm{\hat\Psi}_{t,r}(\vx_t)\big\|^2\Big]
\end{equation}
Then it gives:
\begin{equation}
\begin{aligned}
& \frac{d}{dt} \E_{\vx_t}\Big[\big\|\bm{\Psi}_{t,r}(\vx_t) - \bm{\hat\Psi}_{t,r}(\vx_t)\big\|^2\Big]\\
& = \E_{\vx_t}\Big[2\Big(\bm{\Psi}_{t,r}(\vx_t) - \bm{\hat\Psi}_{t,r}(\vx_t)\Big)\cdot\Big(\partial_t\bm{\Psi}_{t,r}(\vx_t)+\nabla_{\vx}\bm{\Psi}_{t,r}(\vx_t)\cdot \dot{\vx}_t \\
&\hspace{20em} - \partial_t \bm{\hat\Psi}_{t,r}(\vx_t) - \nabla_{\vx}\bm{\hat\Psi}_{t,r}(\vx_t)\cdot\dot{\vx}_t\Big)\Big]\\
& = \E_{\vx_t}\Big[2\Big(\bm{\Psi}_{t,r}(\vx_t) - \bm{\hat\Psi}_{t,r}(\vx_t)\Big)\cdot\Big(\partial_t\bm{\Psi}_{t,r}(\vx_t)+\nabla_{\vx}\bm{\Psi}_{t,r}(\vx_t)\cdot \vv_t(\vx_t) \\
&\hspace{20em} - \partial_t \bm{\hat\Psi}_{t,r}(\vx_t)-\nabla_{\vx}\bm{\hat\Psi}_{t,r}(\vx_t)\cdot \vv_t(\vx_t)\Big)  \Big] \\
&\geq - \E_{\vx_t}\Big[\big\|\bm{\Psi}_{t,r}(\vx_t) - \bm{\hat\Psi}_{t,r}(\vx_t)\big\|^2\Big] \\
&\hspace{2em} - \E_{\vx_t}\Big[\big\| \partial_t\bm{\Psi}_{t,r}(\vx_t)+\nabla_{\vx}\bm{\Psi}_{t,r}(\vx_t)\cdot \vv_t(\vx_t)  - \partial_t \bm{\hat\Psi}_{t,r}(\vx_t)-\nabla_{\vx}\bm{\hat\Psi}_{t,r}(\vx_t)\cdot \vv_t(\vx_t)\|^2  \Big]
\end{aligned}
\end{equation}
Particularly, we have
\begin{equation}
\begin{aligned}
& \partial_t\bm{\Psi}_{t,r}(\vx_t)+\nabla_{\vx}\bm{\Psi}_{t,r}(\vx_t)\cdot \vv_t(\vx_t) \\
= & \partial_t \big(\vx_t + (r-t)\vu_{t,r}(\vx_t)\big) + \nabla_{\vx}\big(\vx_t + (r-t)\vu_{t,r}(\vx_t)\big)\cdot \vv_t(\vx_t) \\
= & (r-t)\partial_t \vu_{t,r}(\vx_t) - \vu_{t,r}(\vx_t) + \vv_t(\vx_t) + (r-t)\nabla_{\vx}\vu_{t,r}(\vx_t)\cdot\vv_t(\vx_t) \\
= & \vv_t(\vx_t) + (r-t)\frac{d}{dt}\vu_{t,r}(\vx_t) - \vu_{t,r}(\vx_t)
\end{aligned}
\end{equation}
On the other side, taking derivative w.r.t. $t$ on both sides of 
\begin{equation}
(r-t)\vu_{t,r}(\vx_t) = \int_t^r \vv_s(\vx_s)ds
\end{equation}
gives
\begin{equation}
\vv_t(\vx_t) = \vu_{t,r}(\vx_t) - (r-t)\frac{d}{dt}\vu_{t,r}(\vx_t) 
\end{equation}
so we have
\begin{equation}
\partial_t\bm{\Psi}_{t,r}(\vx_t)+\nabla_{\vx}\bm{\Psi}_{t,r}(\vx_t)\cdot \vv_t(\vx_t) = 0
\end{equation}
Similarly, we have 
\begin{equation}
\begin{aligned}
&-\partial_t \bm{\hat\Psi}_{t,r}(\vx_t)-\nabla_{\vx}\bm{\hat\Psi}_{t,r}(\vx_t)\cdot \vv_t(\vx_t) \\
=&-\Big((r-t)\partial_t \hat\vu_{t,r}(\vx_t;\theta) - \hat\vu_{t,r}(\vx_t;\theta) + \vv_t(\vx_t) + (r-t)\nabla_{\vx}\hat\vu_{t,r}(\vx_t;\theta)\cdot\vv_t(\vx_t) \Big) \\
=&-\Big((r-t)\partial_t \hat\vu_{t,r}(\vx_t;\theta^{-}) - \hat\vu_{t,r}(\vx_t;\theta) + \vv_t(\vx_t) + (r-t)\nabla_{\vx}\hat\vu_{t,r}(\vx_t;\theta^{-})\cdot\vv_t(\vx_t) \Big) \\
=& \hat\vu_{t,r}(\vx_t;\theta) - \vu_{t,r}^{\rm tgt}(\vx_t;\theta^{-})
\end{aligned}
\end{equation}

Thus, we have
\begin{equation}
\begin{aligned}
\frac{d}{dt} \E_{\vx_t}\Big[\big\|\bm{\Psi}_{t,r}(\vx_t) - \bm{\hat\Psi}_{t,r}(\vx_t)\big\|^2\Big] &\geq -  \E_{\vx_t}\Big[\big\|\bm{\Psi}_{t,r}(\vx_t) - \bm{\hat\Psi}_{t,r}(\vx_t)\big\|^2\Big] \\
&\hspace{3em}- \E_{\vx_t}\Big[\|\hat\vu_{t,r}(\vx_t;\theta) - \vu_{t,r}^{\rm tgt}(\vx_t;\theta^{-})\big\|^2\Big]
\end{aligned}
\end{equation}
which implies
\begin{equation}
-\frac{d}{dt}\exp{(t)}\E_{\vx_t}\Big[\big\|\bm{\Psi}_{t,r}(\vx_t) - \bm{\hat\Psi}_{t,r}(\vx_t)\big\|^2\Big] \leq \exp{(t)}\E_{\vx_t}\Big[\|\hat\vu_{t,r}(\vx_t;\theta) - \vu_{t,r}^{\rm tgt}(\vx_t;\theta^{-})\big\|^2\Big]
\end{equation}
Note the fact that $\bm{\Psi}_{r,r}(\vx_r) = \bm{\hat\Psi}_{r,r}(\vx_r)$, integrating w.r.t. $t$ from $t$ to $r$ gives:
\begin{equation}
\begin{aligned}
&-\exp{(r)}\E_{\vx_r}\Big[\big\|\bm{\Psi}_{r,r}(\vx_r) - \bm{\hat\Psi}_{r,r}(\vx_r)\big\|^2\Big] + \exp{(t)}\E_{\vx_t}\Big[\big\|\bm{\Psi}_{t,r}(\vx_t) - \bm{\hat\Psi}_{t,r}(\vx_t)\big\|^2\Big] \\
&\hspace{20em} \leq \int_t^r \exp{(s)}\E_{\vx_s}\Big[\|\hat\vu_{s,r}(\vx_s;\theta) - \vu_{s,r}^{\rm tgt}(\vx_s;\theta^{-})\big\|^2\Big] ds \\
&\hspace{3em}\Longleftrightarrow \\
&\E_{\vx_t}\Big[\big\|\bm{\Psi}_{t,r}(\vx_t) - \bm{\hat\Psi}_{t,r}(\vx_t)\big\|^2\Big] \leq \int_t^r \exp{(s-t)}\E_{\vx_s}\Big[\|\hat\vu_{s,r}(\vx_s;\theta) - \vu_{s,r}^{\rm tgt}(\vx_s;\theta^{-})\big\|^2\Big] ds \\
\end{aligned}
\end{equation}
1) Let $t=0$, we have
\begin{equation}
\begin{aligned}
\E_{\vx_0}\Big[\big\|\bm{\Psi}_{0,r}(\vx_0) - \bm{\hat\Psi}_{0,r}(\vx_0)\big\|^2\Big] &\leq \int_0^r \exp{(t)}\E_{\vx_t}\Big[\|\hat\vu_{t,r}(\vx_t;\theta) - \vu_{t,r}^{\rm tgt}(\vx_t;\theta^{-})\big\|^2\Big] \\
&=\E_{p(t|r)}\Bigg[ \frac{\exp{(t)}}{p(t|r)}\E_{p_t(\vx)}\Big[\|\hat\vu_{t,r}(\vx;\theta) - \vu_{t,r}^{\rm tgt}(\vx;\theta^{-})\big\|^2\Big]\Bigg]\\
&=\E_{p(t|r),p_t(\vx)}\Big[\frac{\exp{(t)}}{p(t|r)}\|\hat\vu_{t,r}(\vx;\theta) - \vu_{t,r}^{\rm tgt}(\vx;\theta^{-})\big\|^2\Big]\\
\end{aligned}
\end{equation}
Notes that
\begin{equation}
W_2^2(p_{0,r},\hat p_{0,r}) \leq \E_{p_0(\vx)}\Big[\big\|\bm{\Psi}_{0,r}(\vx) - \bm{\hat\Psi}_{0,r}(\vx)\big\|^2\Big]= \E_{\vx_0}\Big[\big\|\bm{\Psi}_{0,r}(\vx_0) - \bm{\hat\Psi}_{0,r}(\vx_0)\big\|^2\Big]
\end{equation}
because the left-hand side takes the infimum over all possible couplings, while the right-hand side corresponds to a specific coupling.

